Online covariance estimation for stochastic gradient descent under Markovian sampling

We investigate the online overlapping batch-means covariance estimator for Stochastic Gradient Descent (SGD) under Markovian sampling. Convergence rates of order $O\big(\sqrt{d}\,n^{-1/8}(\log n)^{1/4}\big)$ and $O\big(\sqrt{d}\,n^{-1/8}\big)$ are established under state-dependent and state-independent Markovian sampling, respectively, where $d$ is the dimensionality and $n$ denotes observations or SGD iterations. These rates match the best-known convergence rate for independent and identically distributed (i.i.d) data. Our analysis overcomes significant challenges that arise due to Markovian sampling, leading to the introduction of additional error terms and complex dependencies between the blocks of the batch-means covariance estimator. Moreover, we establish the convergence rate for the first four moments of the $\ell_2$ norm of the error of SGD dynamics under state-dependent Markovian data, which holds potential interest as an independent result. Numerical illustrations provide confidence intervals for SGD in linear and logistic regression models under Markovian sampling. Additionally, our method is applied to the strategic classification with logistic regression, where adversaries adaptively modify features during training to affect target class classification.

==> jasa_coverletter_preamble.tex <==


% FONTS
\usepackage[T1]{fontenc}

% Import MathDesign (this brings along Bitstream Charter)
% http://www.ctan.org/tex-archive/fonts/mathdesign/
\usepackage[bitstream-charter]{mathdesign}
\usepackage{amsmath}
\usepackage[scaled=0.92]{PTSans}
\usepackage{inconsolata}

% GEOMETRY
\usepackage[
  paper  = letterpaper,
  left   = 1.5in,
  right  = 1.5in,
  top    = 1.0in,
  bottom = 1.0in,
  ]{geometry}

% COLOR
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}

% BIBLIOGRAPHY
\usepackage{natbib}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=Violet}
\hypersetup{linkcolor=black}
\hypersetup{urlcolor=MidnightBlue}

\newcommand{\red}[1]{\textcolor{BrickRed}{\textbf{#1}}}
\pagenumbering{gobble}


==> outlineforSnSlemma.tex <==
\ar{add explanation}
\begin{proof}[Proof outline for Lemma~\ref{lm:SntideSerrorbound}]
%\textbf{Bound on $\expec{\|\tS_n-S\|_2}{}$}\\
Unlike $\iid$ noise, $\tS_n$ is not an unbiased estimator of $S$. So first we establish a bound on the bias term. Since $\te_k$ is a martingale difference sequence, we have 
\begin{align*}
    \expec{\tS_n}{}=&\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\expec{\left(\sum_{k=t_i}^i\te_k\right)\left(\sum_{k=t_i}^i\te_k\right)^\top}{}\\
    =&\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\sum_{k=t_i}^i\expec{\te_k\te_k^\top}{}.\numberthis\label{eq:ekekequaltoSmain}
\end{align*}
Now it can be shown that, 
\iffalse
we have,
\begin{align*}
    &\expec{\te_k\te_k^\top}{}\\
    =&\expec{\left(e'_k+(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})\right)\left(e'_k+(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})\right)^\top}{}\\
    =&\expec{e'_k{e'_k}^\top}{}+\expec{\underbrace{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1}){e'_k}^\top}_{T_{1,k}}}{}+\expec{\underbrace{e'_k(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})^\top}_{T_{2,k}}}{}\\
    &+\expec{\underbrace{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})^\top}_{T_{3,k}}}{}.\numberthis\label{eq:t1t2t3decompmain}
\end{align*}
Now, observe that,
\begin{align*}
    \expec{T_{1,k}}{}=&\expec{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1}){e'_k}^\top}{}\\
    =&\expec{\expec{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1}){e'_k}^\top|\cF_{k-1}}{}}{}\\
    =&\expec{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})(\expec{u(\theta^*,x_k)|\cF_{k-1}}{}-P_{\theta^*} u(\theta^*,x_{k-1}))^\top}{}\\
    =&-\expec{T_{3,k}}{}.
\end{align*}
Similarly, 
\begin{align*}
    \expec{T_{2,k}}{}=-\expec{T_{3,k}}{}.
\end{align*}
Then,
\fi
\begin{align*}
    \expec{\te_k\te_k^\top}{}
    =\expec{e'_k{e'_k}^\top}{}-\expec{T_{3,k}}{},\numberthis\label{eq:ektildeekprimerelmain}
\end{align*}
where $\expec{\norm{T_{3,k}}_2}{}\lesssim \eta_k$.
\iffalse
Note that, using $\expec{T_{3,k}}{}\succcurlyeq 0$, Assumption \ref{as:liangasA3}, and \cs inequality we have the following bound on $\norm{\expec{T_{3,k}}{}}_2$.
\begin{align*}
    \expec{\norm{T_{3,k}}_2}{}= &\expec{\norm{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})^\top}_2}{}\\
    =&\expec{\norm{(P_{\theta^*} -P_{\theta_{k-1}}) u(\theta^*,x_{k-1})}_2^2}{}\\
    \leq &\expec{\norm{\theta_{k-1}-\theta^*}_2^2 V(x_{k-1})^2}{}\\
    \leq & \sqrt{\expec{\norm{\theta_{k-1}-\theta^*}_2^4}{}\expec{V(x_{k-1})^4}{}}\\
    \lesssim & \eta_k \numberthis\label{eq:T3kbound}
\end{align*}
\fi
Now let us concentrate on the term $\expec{e'_k{e'_k}^\top}{}$. Note that this is function of $x_k$, and $x_{k-1}$. For convenience let us write $e'_k{e'_k}^\top=\mathcal{A}(x_{k-1},x_k)$. Here we make two observations. Firstly, the distance $\norm{\theta_{k+1}-\theta_{k}}_2$ between two consecutive iterates is of the order of the step-size $\eta_{k+1}$, and secondly, $\expec{\norm{\theta_k-\theta^*}_2}{}=O(\sqrt{\eta_k})$. Combining these two facts, one can deduce that for small enough $b_0$, the expectation of the variables $\mathcal{A}(x_{k-1},x_k)$, and $\mathcal{A}(x_{k-1}',x_k')$ are close, where,
\begin{align*}
    &\mathcal{A}(x_{k-1},x_k)\sim P_{\theta_0}(x_0)P_{\theta_1}(x_1|x_0)\cdots P_{\theta_{k-1}}(x_{k}|x_{k-1})\\
    &\mathcal{A}(x_{k-1}',x_k')\sim P_{\theta_0}(x_0)P_{\theta_1}(x_1|x_0)\cdots P_{\theta_{k-b_0-1}}(x_{k-b_0}|x_{k-b_0-1})P_{\theta^*}(x_{k-b_0+1}'|x_{k-b_0})\cdots P_{\theta^*}(x_{k}'|x_{k-1}').
\end{align*}
 But, by Assumption~\ref{as:liangasA3}, we have that for a fixed $\theta$ the chain mixes exponentially fast to $\pi_\theta$. Now, for a proper choice of $b_0$, $\expec{\mathcal{A}(x_{k-1}',x_k')}{}$ is close to $\expec{\mathcal{A}(\hat{x}_{k-1},\hat{x}_k)}{}$ where $\hat{x}_{k-1}\sim\pi_{\theta^*}$, and $\hat{x}_k$ is obtained from $\hat{x}_{k-1}$ after transition according to the transition operator $P_{\theta^*}$. This implies $\expec{\mathcal{A}(\hat{x}_{k-1},\hat{x}_k)}{}=S$. 

Now let us define another sequence $\{x'_i\}$ as follows: $x'_i=	x_i$  for $ i=1,2,\cdots,k-b_0$, and $x'_{k-b_0+j}$, $j=1,\cdots,b_0$ are obtained after applying transition operator $P_{\theta^*}$ to $x'_{k-b_0}$ $j$ times. Let $\hat e_k\coloneqq u(\theta^*,x'_k)-P_{\theta^*}u(\theta^*,x'_{k-1})$.
Note that,
\iffalse
\begin{align*}
    &\expec{\hat e_k\hat e_k^\top}{}=\int \mathcal{A}(x_{k-1},x_k)P_{\theta^*}(x_{k-1},x_k)P_{\theta^*}(x_{k-2},x_{k-1})\cdots P_{\theta_{k-b_0-1}}(x_{k-b_0-1},x_{k-b_0})\cdots P_{\theta_0}(x_0)dx_kdx_{k-1}\cdots dx_0\\
    &\expec{e_k' {e'_k}^\top}{}=\int \mathcal{A}(x_{k-1},x_k)P_{\theta_{k-1}}(x_{k-1},x_k)P_{\theta_{k-2}}(x_{k-2},x_{k-1})\cdots P_0(x_0)dx_kdx_{k-1}\cdots dx_0. \numberthis\label{eq:hatekdef}
\end{align*}
In short we write,
\fi
\begin{align*}
    &\expec{\hat e_k\hat e_k^\top}{}=\int \mathcal{A}(x_{k-1},x_k)P_{\theta^*}^{b_0} P_{\theta_{k-b_0-1}}\cdots P_{\theta_0} dx_kdx_{k-1}\cdots dx_0\\
    &\expec{e_k' {e'_k}^\top}{}=\int \mathcal{A}(x_{k-1},x_k)P_{\theta_{k-1}}P_{\theta_{k-2}}\cdots P_{\theta_0} dx_kdx_{k-1}\cdots dx_0.
\end{align*}
Then we can write 
\begin{align*}
   \expec{\hat e_k\hat e_k^\top}{}=\expec{e_k' {e'_k}^\top}{}+\sum_{j=1}^{b_0}\int \mathcal{A}(x_{k-1},x_k)P_{\theta^*}^{b_0-j}(P_{\theta_{k-(b_0-j)}}-P_{\theta^*})P_{\theta_{k-(b_0-j)-1}}\cdots P_{\theta_0} dx_kdx_{k-1}\cdots dx_0.\numberthis\label{eq:ekhatekorimediffmain}
\end{align*}
Now by Assumption~\ref{as:liangasA3}(c) we have,
\begin{align*}
    \norm{P_{\theta^*}^{b_0-j}P_{\theta_{k-(b_0-j)}}P_{\theta_{k-(b_0-j)-1}}\cdots P_{\theta_0}-P_{\theta^*}^{b_0-j+1}P_{\theta_{k-(b_0-j)-1}}\cdots P_{\theta_0}}_{TV}\lesssim \sqrt{\eta_{k-(b_0-j)}}.\numberthis\label{eq:totalvariationmain}
\end{align*}
Using \eqref{eq:totalvariationmain}, we get,
\begin{align*}
    \int \mathcal{A}(x_{k-1},x_k)P_{\theta^*}^{b_0-j}(P_{\theta_{k-(b_0-j)}}-P_{\theta^*})P_{\theta_{k-(b_0-j)-1}}\cdots P_{\theta_0} dx_kdx_{k-1}\cdots dx_0\lesssim \sqrt{\eta_{k-(b_0-j)}}.
\end{align*}
Then from \eqref{eq:ekhatekorimediffmain}, we get,
\begin{align*}
    \expec{e_k' {e'_k}^\top}{}=\expec{\hat e_k\hat e_k^\top}{}-T_{4,k}, \numberthis\label{eq:ekprimeekhatrelmain}
\end{align*}
where 
\begin{align*}
    \norm{T_{4,k}}_2\lesssim \sum_{j=0}^{b_0-1}\sqrt{\eta_{k-j}}.\numberthis\label{eq:T4normboundmain}
\end{align*}
By Assumption~\ref{as:liangasA3}, one has that for each $\theta$, the Markov chain $\{x_k\}_k$ is $V$-uniformly ergodic. Let $\Delta$ denote the joint distribution of $(x'_{k-1},x'_k)$ conditioned on $x_{k-b_0}$, and $\Delta_{\theta^*}$ is the joint distribution $(\hat x_{k-1},\hat x_k)$ where $\hat x_{k-1}\sim\pi_{\theta^*}$, and $\hat x_k$ is obtained by applying the transition operator $P_{\theta^*}$ on $\hat x_{k-1}$. Note that $\expec{\mathcal{A}(\hat x_{k-1},\hat x_k)}{}=S$. One can write $\Delta=P_{\theta^*}P(x'_{k-1})=P_{\theta^*}\pi_{\theta^*}+P_{\theta^*}(P(x'_{k-1})-\pi_{\theta^*})=\Delta_{\theta^*}+P_{\theta^*}(P(x'_{k-1})-\pi_{\theta^*})$. Then, 
\begin{align*}
    \norm{\Delta-\Delta_{\theta^*}}_{TV}=& \norm{P_{\theta^*}(P(x'_{k-1})-\pi_{\theta^*})}_{TV}\\
    =&\int\left(\int P_{\theta^*}(x'_k|x'_{k-1})dx_k\right)(P(x'_{k-1})-\pi_{\theta^*(x'_{k-1})})dx'_{k-1}\\
    \leq & CV(x_{k-b_0})\rho^{b_0},
\end{align*}
for some constant $C>0$, and $0<\rho<1$. 

Then we have, 
\begin{align*}
    \expec{\mathcal{A}(x'_{k-1},x'_k)|x_{k-b_0}}{}=S+T_{5,k}, \numberthis\label{eq:Asrelationmain}
\end{align*}
where $\norm{T_{5,k}}_2\lesssim V(x_{k-b_0})\rho^{b_0}$. Taking expectation on both sides of \eqref{eq:Asrelationmain} with respect to $x_{k-b_0}$ we have,
\begin{align*}
    \expec{\mathcal{A}(x'_{k-1},x'_k)}{}=S+\expec{T_{5,k}}{}, \numberthis\label{eq:Asrelationfinalmain}
\end{align*}
where, $\expec{\norm{T_{5,k}}_2}{}\lesssim \rho^{b_0}$. Choosing $b_0=\ceil{\log \eta_k/\log \rho}$, and from \eqref{eq:T4normboundmain}, we get, 
\begin{align*}
    {\norm{T_{4,k}}_2}\lesssim \eta_k\log k, \quad \expec{\norm{T_{5,k}}_2}{}\lesssim \eta_k. \numberthis\label{eq:T4T5bound}
\end{align*}
Combining \eqref{eq:ektildeekprimerelmain}, \eqref{eq:ekprimeekhatrelmain}, and \eqref{eq:Asrelationfinalmain}, we get,
\begin{align*}
    \expec{\te_k\te_k^\top}{}=S-\expec{T_{3,k}}{}-T_{4,k}+\expec{T_{5,k}}{}.\numberthis\label{eq:ekekdecompmain}
\end{align*}
Then, from \eqref{eq:ekekequaltoSmain}, we get, 
\begin{align*}
    \expec{\tS_n}{}
    =&\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\sum_{k=t_i}^i\expec{\te_k\te_k^\top}{}\\
    =&S+T_6,
\end{align*}
where 
\begin{align}
    \norm{T_6}_2\leq M^{-a\beta}\log M. \label{eq:T6boundmain}
\end{align}
This establishes the bound on the bias term. 
\iffalse
\begin{align*}
    T_6=\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\sum_{k=t_i}^i(\expec{T_{5,k}}{}-\expec{T_{3,k}}{}-T_{4,k}).
\end{align*}
Now, using \eqref{eq:T3kbound}, and \eqref{eq:T4T5bound} we have, 
\begin{align*}
    \norm{T_6}_2\leq & \left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\sum_{k=t_i}^i\norm{\expec{T_{5,k}}{}-\expec{T_{3,k}}{}-T_{4,k}}_2\\
    \lesssim & \left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\sum_{k=t_i}^i \eta_k \log k \\
    \lesssim &\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\sum_{k=t_i}^ik^{-a}\log k\\
    \leq &\log a_M\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{m=1}^M\sum_{i=a_m}^{a_{m+1}-1}l_ia_m^{-a}\\
    \leq &\log a_M\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{m=1}^Mn_m^2a_m^{-a}.
\end{align*}
The last inequality follows from the following fact.
\begin{align*}
    \sum_{i=a_m}^{a_{m+1}-1}l_i \asymp n_m^2.
\end{align*}
Choosing $a_m=\floor{Cm^\beta}$ where $\beta>1/(1-a)$, we have, $n_m\asymp m^{\beta-1}$, and,
\begin{align*}
    \log a_M\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{m=1}^Mn_m^2a_m^{-a}\lesssim M^{-a\beta}\log M.\numberthis\label{eq:expecbkbkboundmain}
\end{align*}
\fi
\iffalse 
\ar{In \eqref{eq:ekekequaltoS}, $\expec{(\tilde{e_k}\tilde{e_k}^\top)}{}$ cannot be written equal to $S$.   $\tilde{e_k}$ is defined in \eqref{eq:tildekdef}. Rather,  $\tilde{e_k}$ should be defined as $\tilde{e_k}=u(\theta^*,x_k^*)-P_{\theta^*}u(\theta^*,x_{k-1}^*)$, where $x_k^*\sim P_{\theta^*}(x_{k-1}^*,\cdot)$ to be able to write $E(\tilde{e_k}\tilde{e_k}^\top) =S$. But this breaks down then proof from \eqref{eq:bkintermed} onwards. Basically how $\expec{e_ke_k^\top}{}$ converges to $\expec{\tilde{e}_k\tilde{e}_k^\top}{}$ is the main question.}\\
\fi

As $\tS_n-S$ is a symmetric matrix, we have,
\begin{align*}
    \expec{\|\tS_n-S\|_2}{}\leq \expec{\sqrt{\tr\left(\tS_n-S\right)^2}}{}\leq \sqrt{\tr\expec{\left(\tS_n-S\right)^2}{}}\leq\sqrt{d\norm{\expec{\left(\tS_n-S\right)^2}{}}_2}\numberthis\label{eq:snstr2normrelmain}
\end{align*}
Now,
\begin{align*}
    \expec{\left(\tS_n-S\right)^2}{}=\expec{\tS_n^2}{}+2T_6S-S^2.
\end{align*}
Using \eqref{eq:T6boundmain}, we have, 
\begin{align*}
    \norm{2T_6S}_2\lesssim M^{-a\beta}\log M. \numberthis\label{eq:sn2decompmidmain}
\end{align*}
Now we will show that $\expec{\tS_n^2}{}-S^2$ is small. 

Similar to equation (45) in \cite{zhu2021online}, the following preliminary decomposition takes place for $\expec{\tS_n^2}{}$. 
\begin{align*}
    \tS_n^2=\left(\sum_{i=1}^nl_i\right)^{-2}(R_1+R_2), 
\end{align*}
where,
\begin{align*}
    R_1=&\sum_{m=1}^{M-1}\sum_{i=a_m}^{a_{m+1}-1}\left[2\sum_{j=a_m}^{i-1}\sum_{a_m\leq p_1\neq p_2\leq j}\left(\te_{p_1}\te_{p_1}^\top \te_{p_1}\te_{p_2}^\top+\te_{p_1}\te_{p_1}^\top \te_{p_2}\te_{p_1}^\top\right)+\sum_{a_m\leq p_1\neq p_2\leq i}\left(\te_{p_1}\te_{p_1}^\top \te_{p_1}\te_{p_2}^\top+\te_{p_1}\te_{p_1}^\top \te_{p_2}\te_{p_1}^\top\right)\right]\\
    &+\sum_{i=a_M}^{n}\left[2\sum_{j=a_M}^{i-1}\sum_{a_M\leq p_1\neq p_2\leq j}\left(\te_{p_1}\te_{p_1}^\top \te_{p_1}\te_{p_2}^\top+\te_{p_1}\te_{p_1}^\top \te_{p_2}\te_{p_1}^\top\right)+\sum_{a_M\leq p_1\neq p_2\leq i}\left(\te_{p_1}\te_{p_1}^\top \te_{p_1}\te_{p_2}^\top+\te_{p_1}\te_{p_1}^\top \te_{p_2}\te_{p_1}^\top\right)\right],\numberthis\label{eq:Idef}
\end{align*}
and,
\begin{align*}
    R_2=\sum_{i=1}^n\sum_{j=1}^n\sum_{p=t_i}^i\sum_{q=t_j}^j \te_p\te_p^\top \te_q\te_q^\top.\numberthis\label{eq:IIdef}
\end{align*}
Using equation (46) from \cite{zhu2021online}, we have,
\begin{align*}
    \left(\sum_{i=1}^nl_i\right)^{-2}\norm{\expec{R_1}{}}_2\lesssim M^{-1}.\numberthis\label{eq:R1boundmain}
\end{align*}
Similar to equation (47) in \cite{zhu2021online}, we have,
\begin{align*}
    \norm{\left(\sum_{i=1}^nl_i\right)^{-2}\expec{R_2}{}-S^2}_2\lesssim \left(\sum_{i=1}^{a_{M+1}-1}l_i\right)^{-2}\sum_{m=1}^M\sum_{k=1}^M\sum_{i=a_m}^{a_{m+1}-1}\sum_{j=a_k}^{a_{k+1}-1}\sum_{p=a_m}^i\sum_{q=a_k}^j\norm{\expec{\te_p\te_p^\top \te_q\te_q^\top}{}-S^2}_2.\numberthis\label{eq:IIinitialdecompmain}
\end{align*}
At this point we need a more careful analysis to bound the right hand side of \eqref{eq:IIinitialdecompmain}. Unlike \cite{zhu2021online}, $\expec{\te_p\te_p^\top \te_q\te_q^\top}{}\neq S^2$ when $p$ and $q$ belong to different blocks since $S$ is defined as the asymptotic covariance of a martingale-difference sequence derived from a $\theta_k$-dependent Markov chain whereas $S$ is the covariance of an $\iid$ sequence in \cite{zhu2021online}. So, now we establish a bound on this bias. 

We decompose \eqref{eq:IIinitialdecompmain} into two terms.  
\begin{enumerate}
    \item $p$ and $q$ belong to either same block or neighboring blocks, i.e., $\abs{m-k}\leq 1$.
    \item $p$ and $q$ are at least $1$ block apart, i.e., $\abs{m-k}> 1$.
\end{enumerate}
In the first component, the correlation among the terms are high. So we just use a constant bound for these terms. In the second component, using the fact that the blocks are separated enough, we show that the correlation between the blocks are small. Then we show that these terms $\te_p\te_p^\top \te_q\te_q^\top$ can estimate $S^2$ with small bias.\\
\textbf{Case I. $\abs{m-k}\leq 1$.}
\begin{align*}
    R_3\coloneqq \mathop{\sum_{m=1}^M\sum_{k=1}^M}\limits_{\abs{m-k}\leq 1}\sum_{i=a_m}^{a_{m+1}-1}\sum_{j=a_k}^{a_{k+1}-1}\sum_{p=a_m}^i\sum_{q=a_k}^j \norm{\expec{\te_p\te_p^\top \te_q\te_q^\top}{}-S^2}_2. \numberthis\label{eq:IIIeeeedefmain}
\end{align*}
By Lemma~\ref{lm:noisedecompmain} we have, $\norm{\expec{\te_p\te_p^\top \te_q\te_q^\top}{}}_2\leq C$ for some constant $C>0$. When $n_m\asymp m^{\beta-1}$, we have $$n_m^2+n_{m+1}^2+n_{m-1}^2\leq (4^\beta+2)n_m^2.$$ 
Then, using $\sum_{i=a_m}^{a_{m+1}-1}l_i\lesssim n_m^2$, we have, 
\iffalse
\begin{align*}
    R_3\lesssim \mathop{\sum_{m=1}^M\sum_{k=1}^M}\limits_{\abs{m-k}\leq 1}\sum_{i=a_m}^{a_{m+1}-1}\sum_{j=a_k}^{a_{k+1}-1}l_il_j
    \lesssim \mathop{\sum_{m=1}^M\sum_{k=1}^M}\limits_{\abs{m-k}\leq 1}n_m^2n_k^2
    \lesssim \sum_{m=1}^M n_m^4
    \lesssim M^{4\beta-3}.\numberthis\label{eq:diffless1numbound}
\end{align*}
We also have, 
\begin{align*}
    \left(\sum_{i=1}^{a_{M+1}-1}l_i\right)^{2}=\left(\sum_{m=1}^{M}\sum_{i=a_m}^{a_{m+1}-1}l_i\right)^{2}\asymp \left(\sum_{m=1}^{M}n_m^2\right)^{2}\asymp M^{4\beta-2}.\numberthis\label{eq:li2bound}
\end{align*}
Combining \eqref{eq:diffless1numbound}, and \eqref{eq:li2bound}, we get, 
\fi
\begin{align*}
   \left(\sum_{i=1}^{a_{M+1}-1}l_i\right)^{-2} R_3\lesssim M^{-1}.\numberthis\label{eq:R3boundmain}
\end{align*}
\textbf{Case II. $\abs{m-k}> 1$.}
Let
\begin{align*}
    R_4\coloneqq \mathop{\sum_{m=1}^M\sum_{k=1}^M}\limits_{\abs{m-k}> 1}\sum_{i=a_m}^{a_{m+1}-1}\sum_{j=a_k}^{a_{k+1}-1}\sum_{p=a_m}^i\sum_{q=a_k}^j \norm{\expec{\te_p\te_p^\top \te_q\te_q^\top}{}-S^2}_2. \numberthis\label{eq:IIIeeeedefmain}
\end{align*}
Let us assume $k\leq m-2$. Then, 
\begin{align*}
    \expec{\te_p\te_p^\top \te_q\te_q^\top|\cF_{a_{m-1}-1}}{}=\expec{\te_p\te_p^\top |\cF_{a_{m-1}-1}}{}\te_q\te_q^\top.
\end{align*}
Now using similar arguments as in \eqref{eq:ektildeekprimerelmain}-\eqref{eq:ekekdecompmain}, we show that the bias to estimate $S^2$ is small, i.e.,
\begin{align*}
    \norm{\expec{\te_p\te_p^\top \te_q\te_q^\top}{}-S^2}_2
    \lesssim & \sqrt{\eta_p}\log p+\sqrt{\eta_q}\log q.
\end{align*}
\iffalse
Similar to \eqref{eq:t1t2t3decomp}, we get,
\begin{align*}
    \expec{\te_p\te_p^\top |\cF_{a_{m-1}-1}}{}=\expec{e_p'{e_p'}^\top |\cF_{a_{m-1}-1}}{}-\expec{T_{3,p}|\cF_{a_{m-1}-1}}{}.\numberthis\label{eq:eptildeprimecondn}
\end{align*}
Now, for consider the sequence $\{\hat{e}_p\}_p$ defined similarly as in \eqref{eq:hatekdef}. We will choose $b_0$ such that $b_0\leq n_{m-1}+1$. Then similar to \eqref{eq:ekprimeekhatrel}, we have, 
\begin{align*}
    \expec{e_p'{e_p'}^\top|\cF_{a_{m-1}-1}}{}=\expec{\hat e_p\hat e_p^\top|\cF_{a_{m-1}-1}}{}-T'_{4,p}, \numberthis\label{eq:ekprimeekhatrelcond}
\end{align*}
where 
\begin{align*}
    T'_{4,p}=\sum_{j=1}^{b_0}\int \mathcal{A}(x_{p-1},x_p)P_{\theta^*}^{b_0-j}(P_{\theta_{p-(b_0-j)}}-P_{\theta^*})P_{\theta_{p-(b_0-j)-1}}\cdots P_{a_{m-1}} dx_pdx_{p-1}\cdots dx_{a_{m-1}},
\end{align*}
and
\begin{align*}
    \norm{T'_{4,p}}_2=\sum_{j=1}^{b_0}\sqrt{\eta_{p-j}}.\numberthis\label{eq:T4pbound}
\end{align*}
Similar to \eqref{eq:Asrelationfinal}, we have,
\begin{align*}
    \expec{\mathcal{A}(x'_{p-1},x'_p)|\cF_{a_{m-1}-1}}{}=S+\expec{T_{5,p}|\cF_{a_{m-1}-1}}{}, \numberthis\label{eq:Asrelationfinalcondn}
\end{align*}
where $\norm{T_{5,p}}_2\leq V(x_{p-b_0})\rho^{b_0}$.
Combining \eqref{eq:eptildeprimecondn}, \eqref{eq:ekprimeekhatrelcond}, and \eqref{eq:Asrelationfinalcondn}, we have,
\begin{align*}
    \expec{\te_p\te_p^\top |\cF_{a_{m-1}-1}}{}=S+\expec{T_{5,p}|\cF_{a_{m-1}-1}}{}-T'_{4,p}-\expec{T_{3,p}|\cF_{a_{m-1}-1}}{}.\numberthis\label{eq:eptildeScondn}
\end{align*}
Then, we have, 
\begin{align*}
    \expec{\te_p\te_p^\top \te_q\te_q^\top}{}=S\expec{\te_q\te_q^\top}{}+\expec{\left(T_{5,p}-T'_{4,p}-T_{3,p}\right)\te_q\te_q^\top}{}.
\end{align*}
Similar to \eqref{eq:ekekdecomp}, we have
\begin{align*}
    \expec{\te_q\te_q^\top}{}=S-\expec{T_{3,q}}{}-T_{4,q}+\expec{T_{5,q}}{}.\numberthis\label{eq:ekekdecompcondn}
\end{align*} 
We also have, similar to \eqref{eq:T3kbound},  for \textcolor{blue}{$\alpha_0\geq 8$},
\begin{align*}
    \expec{\norm{T_{3,p}}_2^\frac43}{}\leq \sqrt{\expec{\norm{\theta_{p-1}-\theta^*}_2^4\expec{V(x_{p-1})^8}{}}{}}\lesssim\eta_p.
\end{align*}
Then, 
\begin{align*}
    &\norm{\expec{\te_p\te_p^\top \te_q\te_q^\top}{}-S^2}_2\\
    \leq&\norm{\expec{\left(T_{5,p}-T'_{4,p}-T_{3,p}\right)\te_q\te_q^\top}{}}_2+\norm{S\left(\expec{T_{3,q}}{}+T_{4,q}-\expec{T_{5,q}}{}\right)}_2\\
    \leq & \expec{\norm{\left(T_{5,p}-T'_{4,p}-T_{3,p}\right)}_2\norm{\te_q\te_q^\top}_2}{}+\norm{S}_2\norm{\left(\expec{T_{3,q}}{}+T_{4,q}-\expec{T_{5,q}}{}\right)}_2\\
    \lesssim & \sqrt{\expec{\norm{\left(T_{5,p}-T'_{4,p}\right)}_2^2{}}{}\expec{\norm{\te_q\te_q^\top}_2^2}{}}+\expec{\norm{T_{3,p}}_2^\frac43}{}\expec{\norm{\te_q\te_q^\top}_2^4}{}+\sum_{j=0}^{b_0-1}\sqrt{\eta_{q-j}}\\
    \lesssim & \sum_{j=0}^{b_0-1}\sqrt{\eta_{p-j}}+\sum_{j=0}^{b_0-1}\sqrt{\eta_{q-j}}\\
    \lesssim & \sqrt{\eta_p}\log p+\sqrt{\eta_q}\log q.
\end{align*}
\fi
Then, using $a_m\asymp m^\beta$, and $n_m\asymp (m+1)^{\beta-1}$, we have, 
\iffalse
\begin{align*}
    R_4\lesssim &\mathop{\sum_{m=1}^M\sum_{k=1}^M}\limits_{\abs{m-k}> 1}\sum_{i=a_m}^{a_{m+1}-1}\sum_{j=a_k}^{a_{k+1}-1}\sum_{p=a_m}^i\sum_{q=a_k}^j \left(\sqrt{\eta_p}\log p+\sqrt{\eta_q}\log q\right)\\
    \lesssim & \mathop{\sum_{m=1}^M\sum_{k=1}^M}\limits_{\abs{m-k}> 1} \left(n_k^2\sum_{i=a_m}^{a_{m+1}-1}\sum_{p=a_m}^i\sqrt{\eta_p}\log p+n_m^2\sum_{j=a_k}^{a_{k+1}-1}\sum_{q=a_k}^j\sqrt{\eta_q}\log q\right)\\
    \lesssim & \sum_{m=1}^M\sum_{k=1}^M\left(n_k^2n_m^2\left(a_m^{-\frac{a}{2}}\log a_{m+1}+a_k^{-\frac{a}{2}}\log a_{k+1}\right)\right)\\
    \lesssim & M^{2+4(\beta-1)-\frac{a\beta}{2}}\log M.
\end{align*}
Using \eqref{eq:li2bound} we have,
\fi
\begin{align*}
    \left(\sum_{i=1}^{a_{M+1}-1}l_i\right)^{-2}R_4\lesssim M^{-\frac{a\beta}{2}}\log M.\numberthis\label{eq:IVboundeeeemain}
\end{align*}
So, combining \eqref{eq:snstr2normrelmain}, \eqref{eq:sn2decompmidmain}, \eqref{eq:R1boundmain}, \eqref{eq:R3boundmain}, and \eqref{eq:IVboundeeeemain}, we get,
\begin{align*}
    \expec{\|\tS_n-S\|_2}{}\leq M^{-\frac{a\beta}{4}}\sqrt{d\log M}+\sqrt{\frac{d}{M}}+M^{-\frac{a\beta}{2}}\sqrt{d\log M}.\numberthis\label{eq:SntideSerrorbound}
\end{align*}
\end{proof}
\begin{proof}[Proof outline of Lemma~\ref{lm:esntildesndiffprelim}]
%\textbf{Bound on $\expec{\norm{\tS_n-S_n}_2}{}$}\\
Define $b_k=e_k-\te_k$. Note that $b_k$ is a martingale difference sequence as well.
\iffalse
First let us establish a bound on $\expec{\|b_k\|_2^2}{}$ which will be crucial to establish a bound on $\expec{\norm{\tS_n-S_n}_2}{}$.
Then,
\begin{align*}
    &\expec{\|b_k\|_2^2}{}\\
    =&\expec{\|e_k-\te_k\|_2^2}{}\\
    =&\expec{\|u(\tt_{k-1},x_{k})-u(\theta^*,x_k)-(P_{\tt_{k-1}} u(\tt_{k-1},x_{k-1})-P_{\theta^*} u(\theta^*,x_{k-1}))\|_2^2}{}\\
    \lesssim & \expec{\|u(\tt_{k-1},x_{k})-u(\theta^*,x_k)\|_2^2}{}+\expec{\|(P_{\tt_{k-1}} u(\tt_{k-1},x_{k-1})-P_{\tt^*} u(\theta^*,x_{k-1}))\|_2^2}{}\\
    \leq& \expec{\left(V(x_k)^2+V(x_{k-1})^2\right)\|\tt_{k-1}-\theta^*\|_2^{2}}{}. \numberthis\label{eq:bkintermed}
\end{align*}
\fi
Now, using Lemma~\ref{lm:expecconviter}, we have,
\begin{align*}
    \expec{\|b_k\|_2^2}{}\lesssim \expec{\|\tt_{k-1}-\theta^*\|_2^{2}}{}\leq \eta_k\leq k^{-a}\numberthis\label{eq:bkboundmain}
\end{align*}
\iffalse
\begin{lemma}
\begin{align}
    \expec{\|\tt_{k}-\theta^*\|^2_2}{}\leq& O(\eta_{k})
\end{align}
\end{lemma}
\begin{proof}
Choosing $\eta_{k+1}\leq 1/(2L_G)$, we have,
\begin{align*}
    f(\theta_{k+1})\leq& f(\theta_k)+\nabla f(\theta_k)^\top (\theta_{k+1}-\theta_{k})+\frac{L_G}{2}\|\theta_{k+1}-\theta_k\|_2^2\\
    =&f(\theta_k)-\eta_{k+1}\nabla f(\theta_k)^\top \nabla F(\theta_{k},x_{k+1})+\frac{L_G\eta_{k+1}^2}{2}\|\nabla F(\theta_{k},x_{k+1})\|_2^2\\
    =&f(\theta_k)-\eta_{k+1}\nabla f(\theta_k)^\top \left(\nabla f(\theta_{k})+\xi_{k+1}(\theta_k,x_{k+1})\right)+\frac{L_G\eta_{k+1}^2}{2}\|\nabla f(\theta_{k})+\xi_{k+1}(\theta_k,x_{k+1})\|_2^2\\
    \leq &f(\theta_k)-\eta_{k+1}\|\nabla f(\theta_k)\|_2^2-\eta_{k+1}\nabla f(\theta_k)^\top \left(u(\theta_k,x_{k+1})-P_{\theta_k} u(\theta_k,x_{k+1})\right)\\
    &+L_G\eta_{k+1}^2\left(\|\nabla f(\theta_{k})\|_2^2+\|\xi_{k+1}(\theta_k,x_{k+1})\|_2^2\right)\\
    \leq &f(\theta_k)-\eta_{k+1}\mu( f(\theta_k)-f(\theta^*))-\eta_{k+1}\nabla f(\theta_k)^\top \left(u(\theta_k,x_{k+1})-P_{\theta_k} u(\theta_k,x_{k+1})\right)\\
    &+L_G\eta_{k+1}^2\|\xi_{k+1}(\theta_k,x_{k+1})\|_2^2
\end{align*}
Taking expectation conditioned on $\mathcal{F}_k$, we have,
\begin{align*}
    \expec{f(\theta_{k+1})-f(\theta^*)|\cF_k}{}\leq& (1-\eta_{k+1}\mu)\left(f(\theta_{k})-f(\theta^*)\right)+L_G\eta_{k+1}^2\sigma^2\\
    \expec{f(\theta_{k+1})-f(\theta^*)}{}\leq& (1-\eta_{k+1}\mu)\expec{f(\theta_{k})-f(\theta^*)}{}+L_G\eta_{k+1}^2\sigma^2\\
    \expec{f(\theta_{k+1})-f(\theta^*)}{}\leq& O(\eta_{k+1})\\
    \expec{\|\theta_{k+1}-\theta^*\|^2_2}{}\leq& O(\eta_{k+1})
\end{align*}

\fi
It is easy to show that,
\begin{align*}
    \expec{\norm{\tS_n-S_n}_2}{}\lesssim& \left((d/M)^{1/4}+C\right)\sqrt{\expec{\norm{\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\left(\sum_{k=t_i}^ib_k\right)\left(\sum_{k=t_i}^ib_k\right)^\top}_2}{}}\\
    &+\expec{\norm{\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\left(\sum_{k=t_i}^ib_k\right)\left(\sum_{k=t_i}^ib_k\right)^\top}_2}{}\numberthis\label{eq:esntildesndiffprelim}
\end{align*}
Then we establish the following bound which completes the proof. Since $b_k$ is a martingale difference sequence, using \eqref{eq:bkboundmain} for $a_m\leq i<a_{m+1}$ we have,
\begin{align*}
    \expec{\norm{\left(\sum_{i=1}^nl_i\right)^{-1}\sum_{i=1}^n\left(\sum_{k=t_i}^ib_k\right)\left(\sum_{k=t_i}^ib_k\right)^\top}_2}{}\lesssim M^{-a\beta}.
\end{align*}
\end{proof}
\end{proof}

==> slowexplanation.tex <==
\subsection{Why state-dependent has to be slow}
In this section, we shed light on why a slower rate of convergence for state-dependent Markov noise is expected. Consider the following problem where the goal is to estimate $\theta^*\in\mathbb{R}$ from noisy observations $\{y_k\}_k$ where the noise $\{\vartheta_{k}\}_k$ is a state-dependent Markov chain. 
\begin{align*}
    y_{k+1}=\theta^*+\vartheta_{k+1} \qquad k=1,2,3,\cdots.
\end{align*}
In this case, one may not recover $\theta^*$ since the noise is dependent on the estimate of $\theta^*$. So similar to strategic classification problem \cite{}, one aims to recover the equilibrium point of the dynamics. Without loss of generality, we assume $\theta^*=0$. In this case, the SGD update is given by, 
\begin{align*}
    \theta_{k+1}=\theta_k-\eta_{k+1}(\theta_k-y_{k+1}).
\end{align*}
When the noise is an $\iid$ or a martingale-difference sequence, or even state-independent exponentially mixing Markov chain, the covariance between the updates $\theta_i$ and $\theta_j$ for $i>j$ decreases exponentially \cite{zhu2021online,polyak1992acceleration}. This is the key behind the faster rate of covariance estimation for the above noise settings as also noted in equation (14), Section 2.1.2 of \cite{zhu2021online}. We will show that, when the noise is a state-dependent Markov chain, the covariance may not decrease exponentially. Consider the following noise model.
\begin{align*}
    \vartheta_{k+1}=B_{k+1}\theta_{k}+\rho_{k+1}\vartheta_k+\omega_{k+1},\numberthis\label{eq:counterex}
\end{align*}
where $\{B_k\}_k$ is a sequence of $\iid$ Bernoulli random variables with $P(B_k=1)=b_k$, $\{\rho_{k}\}_k$ is a decreasing sequence with $0<\rho_{k}<1$ for all $k$, and $\{\omega_k\}_k$ is an $\iid$ $N(0,1)$ sequence independent from $\{B_k\}_k$ and $\theta_k$. Note that this noise dynamics satisfy Assumption~\ref{as:liangasA3}. \ar{todo : assumption verification= irreducible, aperiodic, minorization, drift via $V(\vartheta)=\norm{\vartheta}_2^2+1$}

The joint dynamics of $(\theta_k,\vartheta_k)$ can be written as,
\begin{align*}
    \begin{bmatrix}\theta_{k+1}\\ \vartheta_{k+1}\end{bmatrix}=A_{k+1}\begin{bmatrix}\theta_{k}\\ \vartheta_{k}\end{bmatrix}+\begin{bmatrix}\eta_{k+1}\\ 1\end{bmatrix}\omega_{k+1},
\end{align*}
where $$A_{k+1}=\begin{bmatrix}1-\eta_{k+1}+\eta_{k+1}B_{k+1} & \eta_{k+1}\rho_{k+1}\\ B_{k+1}& \rho_{k+1}\end{bmatrix}.$$
Then, for $k>j>1$ we have, 
\begin{align*}
    \begin{bmatrix}\theta_{k}\\ \vartheta_{k}\end{bmatrix}=\prod_{i=j+1}^kA_{i}\begin{bmatrix}\theta_{j}\\ \vartheta_{j}\end{bmatrix}+\sum_{l=j+1}^{k-1}\left(\prod_{i=l+1}^{k}A_i\right)\begin{bmatrix}\eta_{l}\\ 1\end{bmatrix}\omega_l+\begin{bmatrix}\eta_{k}\\ 1\end{bmatrix}\omega_k,
\end{align*}
Using that $\{\omega_k\}_k$, and $\{B_k\}_k$ are independent, and $\expec{\omega_k}{}=0$, we have, 
\begin{align*}
    \expec{\begin{bmatrix}\theta_{k}\\ \vartheta_{k}\end{bmatrix}\begin{bmatrix}\theta_{j}\\ \vartheta_{j}\end{bmatrix}^\top}{}=\expec{\left(\prod_{i=j+1}^kA_{i}\right)}{}\expec{\begin{bmatrix}\theta_{j}\\ \vartheta_{j}\end{bmatrix}\begin{bmatrix}\theta_{j}\\ \vartheta_{j}\end{bmatrix}^\top}{}=\left(\prod_{i=j+1}^k\expec{A_{i}}{}\right)\expec{\begin{bmatrix}\theta_{j}\\ \vartheta_{j}\end{bmatrix}\begin{bmatrix}\theta_{j}\\ \vartheta_{j}\end{bmatrix}^\top}{}.
\end{align*}
We have, 
\begin{align*}
    \expec{A_i}{}\coloneqq\bar{A}_i=\begin{bmatrix}1-\eta_{i}+\eta_{i}b_{i} & \eta_{i}\rho_{i}\\ b_{i}& \rho_i\end{bmatrix}.
\end{align*}
Let $\tilde{A}\coloneqq\prod_{i=j+1}^k\expec{A_i}{}$.
Then,
\begin{align*}
    Cov(\theta_k,\theta_j)=\tilde{A}_{11}Var(\theta_j)+\tilde{A}_{12}Cov(\theta_j,\vartheta_j).
\end{align*}
We have the following bound: $\tilde{A}_{11}\geq \prod_{i=j+1}^k(1-\eta_i+\eta_ib_i)$, and $\tilde{A}_{12}/\tilde{A}_{11}\to 0$. 
Then, choosing $b_i=1-\rho_i-i^{a-1}$, $\rho_i=i^{a-1}$, and $\eta_i=i^{-a}$, we get,
\begin{align*}
    \tilde{A}_{11}\geq \prod_{i=j+1}^k\left(1-\eta_i i^{a-1}-\eta_i\rho_i\right)=\prod_{i=j+1}^k\left(1-\frac{2}{i}\right)\geq \exp\left(-\sum_{i=j+1}^k\frac4i\right)\geq \exp\left(-\int_{j}^k\frac4idi\right)=\left(\frac{k}{j}\right)^{-4}
\end{align*}
This shows that the covariance between $\theta_j$ and $\theta_i$ decreases polynomially. 
